Learning Getting-Up Policies for Real-World Humanoid Robots

Automatic fall recovery is a crucial prerequisite before humanoid robots can be reliably deployed. Hand-designing controllers for getting up is difficult because of the varied configurations a humanoid can end up in after a fall and the challenging terrains humanoid robots are expected to operate on. This paper develops a learning framework to produce controllers that enable humanoid robots to get up from varying configurations on varying terrains. Unlike previous successful applications of learning to humanoid locomotion, the getting-up task involves complex contact patterns (which necessitates accurately modeling of the collision geometry) and sparser rewards. We address these challenges through a two-phase approach that induces a curriculum. The first stage focuses on discovering a good getting-up trajectory under minimal constraints on smoothness or speed / torque limits. The second stage then refines the discovered motions into deployable (i.e. smooth and slow) motions that are robust to variations in initial configuration and terrains. We find these innovations enable a real-world G1 humanoid robot to get up from two main situations that we considered: a) lying face up and b) lying face down, both tested on flat, deformable, slippery surfaces and slopes (e.g., sloppy grass and snowfield). This is one of the first successful demonstrations of learned getting-up policies for human-sized humanoid robots in the real world.

==> tables/domain_rand.tex <==
\begin{table}[ht!]
\caption{\textbf{Range of dynamics randomization.} This includes simulated dynamics randomization, external perturbations, and terrain variations, which are crucial for sim-to-real transfer, robustness, and generalization.}
\label{table:dr}
\centering
\renewcommand{\arraystretch}{1.3} 
\begin{tabular}{l c}
\toprule[0.95pt]
\textbf{Term} & \textbf{Value} \\
\midrule[0.6pt]
\multicolumn{2}{l}{\textit{\textbf{Dynamics Randomization:}}} \\
\midrule[0.6pt]
Friction & $\mathcal{U}(0.2, 1.1)$ \\
Base CoM offset & $\mathcal{U}(-0.1, 0.1) \text{ m}$ \\
Link mass & $\mathcal{U}(0.7, 1.3) \times \text{default} \text{ kg}$ \\
P Gain & $\mathcal{U}(0.75, 1.25) \times \text{default}$ \\
D Gain & $\mathcal{U}(0.75, 1.25) \times \text{default}$ \\
Torque RFI~\cite{MinimalDyamicsRandomization24} & $0.1 \times \text{Torque Limit} \text{ N}\cdot\text{m}$ \\
Control delay & $\mathcal{U}(20, 60) \text{ ms}$ \\
\midrule[0.6pt]
\multicolumn{2}{l}{\textit{\textbf{External Perturbation:}}} \\
\midrule[0.6pt]
Push robot & $\text{interval} = 5s$, $v_{xy} = 1 \text{ m/s}$ \\
\midrule[0.6pt]
\multicolumn{2}{l}{\textit{\textbf{Randomized Terrain:}}} \\
\midrule[0.6pt]
Terrain type & Flat, rough, slope \\
\bottomrule[0.95pt]
\end{tabular}
\end{table}


==> tables/training_recipe.tex <==
\begin{table}[ht!]
\caption{\textbf{Training recipe of \ours.} 
}
\label{table:training_recipe}
\centering
\renewcommand{\arraystretch}{1.3} % Adjust row spacing
\begin{tabular}{l c c}
 & \texttt{Stage I} & \texttt{Stage II}\\
\toprule[0.95pt]
Config &  & \\
optimizer \\
\bottomrule[0.95pt]
\end{tabular}
\end{table}
